Recursive Scaling in Masked Diffusion Models

Masked diffusion models (MDMs) generate sequences by iteratively refining a partially masked state and committing tokens in parallel. We introduce recursion in MDMs and propose new Recursive Masked Diffusion Models (R-MDMs), which apply a shared denoising transformer $L$ times within each denoising step, adding recursive depth as an additional compute axis without increasing parameter count. Across structured generation tasks, recursive depth improves quality at fixed parameter budget, matches substantially larger non-recursive models at matched FLOPs, and can reduce the number of denoising steps needed to reach a target quality. We interpret these gains with a dependence--fidelity decomposition of parallel decoding error: recursion refines model marginals at a fixed masked state, whereas denoising steps change that state by committing tokens. Building on this analysis, we propose to treat decoding as a two-axis decision (how many loops to run and which tokens to commit) and show that entropy-guided adaptive rules improve the quality--compute frontier over fixed schedules, transferring across various tasks on Sudoku, Countdown, RNA, and executable math generation. Together, these results establish recursive depth as a practical, complementary test-time scaling mechanism for MDMs.

==> figures/tikz/fig1v2_panel_lattice.tex <==
% ---------------------------------------------------------------------------
%  v2 panel (c) -- Inference on the (step, loop) lattice. Streamlined version of
%  fig1_panel_a: no background, no legend, one commit label, terse axis labels.
%  Origin = first cell of (t=1, l=1); spans x in [\XL, \XR], y in [0.95, -2.0].
% ---------------------------------------------------------------------------
% Title is optional: see the note in fig1v2_panel_idea.tex.
\providecommand{\panelTitleLattice}{(c)\; Inference: two axes of refinement}%
\ifx\panelTitleLattice\empty\else
  \node[ptitle] at (\XL, 0.95) {\panelTitleLattice};
\fi

% axes
\draw[axis, cStep!85] (-0.15, 0.58) -- (4*\cp+1.7, 0.58);
\node[hdr, fill=white, text=cStep!90!black, font=\tiny\sffamily\bfseries, inner xsep=3pt] at (2*\cp+0.75, 0.58)
  {denoising steps $t$ \;--\; commit tokens, the state changes};
\draw[axis, cLoop!90] (-1.05, 0.14) -- (-1.05, -1.64);
\node[hdr, anchor=east, text=cLoop!80!black, font=\tiny\sffamily\bfseries, inner sep=0pt] at (-1.12, -0.75)
  {\rotatebox{90}{recursive loops $\ell$}};
\node[hdr, anchor=east, text=black!45, inner sep=0pt] at (-1.31, -0.75)
  {\rotatebox{90}{state fixed}};

\foreach \t in {1,...,4} {
  \node[hdr] at ({(\t-1)*\cp + 0.75}, 0.30) {$t{=}\t$};
}
\node[hdr, text=cInk] at ({4*\cp + 0.75}, 0.30) {output $x_0$};
\foreach \l in {1,...,4} {
  \node[hdr, anchor=east] at (-0.45, {-(\l-1)*\rp}) {$\ell{=}\l$};
}

% realised forward passes
\foreach \t/\n in {0/4, 1/3, 2/2, 3/1} {
  \fill[cLoop!8, rounded corners=2.5pt] ({\t*\cp-0.21}, 0.2) rectangle ({\t*\cp+1.71}, {-(\n-1)*\rp-0.2});
}

% t=1
\tokstrip{(0, 0)}       {4/15, 1/10, 7/8,  9/20, 2/10, 6/12}
\tokstrip{(0, -\rp)}    {4/45, 1/22, 7/15, 9/50, 2/18, 6/28}
\tokstrip{(0, -2*\rp)}  {4/74, 1/38, 7/22, 9/80, 2/24, 6/42}
\tokstrip{(0, -3*\rp)}  {4/92, 1/48, 7/28, 9/95, 2/28, 6/52}
\foreach \l in {0,1,2} { \draw[loopdown] (0.75, {-\l*\rp - 0.16}) -- (0.75, {-(\l+1)*\rp + 0.16}); }
% t=2
\tokstrip{(\cp, 0)}      {4/-2, 1/55, 7/32, 9/-2, 2/32, 6/62}
\tokstrip{(\cp, -\rp)}   {4/-1, 1/80, 7/42, 9/-1, 2/38, 6/84}
\tokstrip{(\cp, -2*\rp)} {4/-1, 1/94, 7/50, 9/-1, 2/42, 6/95}
\foreach \l in {0,1} { \draw[loopdown] (\cp+0.75, {-\l*\rp - 0.16}) -- (\cp+0.75, {-(\l+1)*\rp + 0.16}); }
\node[ghost] at (\cp+0.75, -3*\rp) {};
% t=3
\tokstrip{(2*\cp, 0)}    {4/-1, 1/-2, 7/68, 9/-1, 2/56, 6/-2}
\tokstrip{(2*\cp, -\rp)} {4/-1, 1/-1, 7/93, 9/-1, 2/66, 6/-1}
\draw[loopdown] (2*\cp+0.75, -0.16) -- (2*\cp+0.75, {-\rp + 0.16});
\node[ghost] at (2*\cp+0.75, -2*\rp) {};
\node[ghost] at (2*\cp+0.75, -3*\rp) {};
% t=4
\tokstrip{(3*\cp, 0)}    {4/-1, 1/-1, 7/-2, 9/-1, 2/94, 6/-1}
\node[ghost] at (3*\cp+0.75, -\rp) {};
\node[ghost] at (3*\cp+0.75, -2*\rp) {};
\node[ghost] at (3*\cp+0.75, -3*\rp) {};
% output
\tokstrip{(4*\cp, 0)}    {4/-1, 1/-1, 7/-1, 9/-1, 2/-2, 6/-1}
\node[font=\scriptsize, text=cLoop!80!black] at (4*\cp+1.92, 0) {\ding{51}};

% commits
\draw[commit] (1.70, -3*\rp) .. controls (2.05, -3*\rp) and (1.95, 0) .. (\cp-0.21, 0);
\draw[commit] (\cp+1.70, -2*\rp) .. controls (\cp+2.05, -2*\rp) and (\cp+1.95, 0) .. (2*\cp-0.21, 0);
\draw[commit] (2*\cp+1.70, -\rp) .. controls (2*\cp+2.05, -\rp) and (2*\cp+1.95, 0) .. (3*\cp-0.21, 0);
\draw[commit] (3*\cp+1.70, 0) -- (4*\cp-0.21, 0);
\node[hdr, text=cStep!90!black, anchor=north west, inner sep=0pt] at (1.62, -3*\rp-0.22) {commit $U_1$ (low entropy)};
\node[hdr, text=black!45, anchor=north west, inner sep=0pt] at (2*\cp+0.2, -3*\rp-0.22) {dashed: loops skipped};

% forward-pass meter
\begin{scope}[shift={(4*\cp-0.1, -0.62)}]
  \node[hdr, anchor=north west, text=cInk, font=\tiny\sffamily\bfseries, inner sep=0pt] at (0, 0) {forward passes\; $\NFE{=}\sum_t\ell_t$};
  \fill[black!12, rounded corners=0.8pt] (0, -0.3) rectangle (1.95, -0.5);
  \node[hdr, anchor=west, text=black!60, inner sep=0pt] at (0.06, -0.4) {fixed $L{=}4$};
  \node[hdr, anchor=east, text=black!60, inner sep=0pt, font=\tiny\sffamily\bfseries] at (1.89, -0.4) {16};
  \fill[cLoop!75, rounded corners=0.8pt] (0, -0.58) rectangle (1.95*10/16, -0.78);
  \node[hdr, anchor=west, text=white, inner sep=0pt] at (0.06, -0.68) {adaptive};
  \node[hdr, anchor=east, text=white, inner sep=0pt, font=\tiny\sffamily\bfseries] at (1.95*10/16-0.06, -0.68) {10};
  \node[hdr, anchor=north west, inner sep=0pt, text=cEnt!90!black] at (0, -0.86) {stop when $\overline{\Delta H}^{(\ell)}_t{<}\lambda$};
\end{scope}

